Reasoning Inconsistencies and How to Mitigate Them in Deep Learning

The recent advancements in Deep Learning models and techniques have led to significant strides in performance across diverse tasks and modalities. However, while the overall capabilities of models show promising growth, our understanding of their internal reasoning processes remains limited, particularly concerning systematic inconsistencies or errors patterns of logical or inferential flaws. These inconsistencies may manifest as contradictory outputs, failure to generalize across similar tasks, or erroneous conclusions in specific contexts. Even detecting and measuring such reasoning discrepancies is challenging, as they may arise from opaque internal procedures, biases and imbalances in training data, or the inherent complexity of the task. Without effective methods to detect, measure, and mitigate these errors, there is a risk of deploying models that are biased, exploitable, or logically unreliable. This thesis aims to address these issues by producing novel methods for deep learning models that reason over knowledge graphs, natural language, and images. The thesis contributes two techniques for detecting and quantifying predictive inconsistencies originating from opaque internal procedures in natural language and image processing models. To mitigate inconsistencies from biases in training data, this thesis presents a data efficient sampling method to improve fairness and performance and a synthetic dataset generation approach in low resource scenarios. Finally, the thesis offers two techniques to optimize the models for complex reasoning tasks. These methods enhance model performance while allowing for more faithful and interpretable exploration and exploitation during inference. Critically, this thesis provides a comprehensive framework to improve the robustness, fairness, and interpretability of deep learning models across diverse tasks and modalities.

==> frontbackmatter/bibliography.tex <==
\chapter{Bibliography}
\vspace{1cm}
\printbibliography[heading=none]

==> frontbackmatter/titlepage.tex <==
% Cover back page
\AddToShipoutPicture*{\TitleWatermark}% adding watermark
\hfill
\vfill
{
	\small
	\textbf{\thesisName} \\
	\textit{\thesisTitle} \\
	\thesisSubject, \thesisDate \\
	Supervisors: \thesisExternalSupervisor\ and \thesisInternalSupervisor \\[1.5em]
	\textbf{\thesisUniversity} \\
	\textit{\thesisFaculty} \\
	\thesisInstitute \\
	\thesisAddress \\
	\thesisPostal\ \thesisCity
}


==> tables/drop_rate.tex <==

\begin{table*}[t]
\centering
\begin{tabular}{@{}clcccccc|c@{}}
\toprule
                                                                                                  & \textbf{}                         & \textbf{bart-l} & \textbf{roberta-l} & \textbf{distilbart} & \textbf{deberta-b} & \textbf{deberta-l} & \textbf{deberta-xl} & Average                  \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}MNLI\end{tabular}}}     & \multicolumn{1}{l|}{1st Dropping} & 90.10\%         & 90.56\%            & 87.17\%             & 88.77\%            & 91.32\%            & 91.44\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 88.89\%         & 89.24\%            & 86.13\%             & 87.07\%            & 89.69\%            & 90.28\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{1.20\%} & \textbf{1.31\%}    & \textbf{1.04\%}     & \textbf{1.70\%}    & \textbf{1.63\%}    & \textbf{1.16\%}     & \textbf{1.34\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}SNLI\end{tabular}}}    & \multicolumn{1}{l|}{1st Dropping} & 87.55\%         & 86.44\%            & 84.37\%             & 84.39\%            & 88.87\%            & 88.54\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 82.78\%         & 81.78\%            & 82.02\%             & 78.89\%            & 83.64\%            & 84.62\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{4.77\%} & \textbf{4.66\%}    & \textbf{2.35\%}     & \textbf{5.50\%}    & \textbf{5.23\%}    & \textbf{3.92\%}     & \textbf{4.41\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ANLI\_r1\end{tabular}}} & \multicolumn{1}{l|}{1st Dropping} & 46.20\%         & 46.40\%            & 41.40\%             & 35.10\%            & 49.70\%            & 53.00\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 45.60\%         & 44.90\%            & 41.10\%             & 34.30\%            & 48.60\%            & 52.00\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{0.60\%} & \textbf{1.50\%}    & \textbf{0.30\%}     & \textbf{0.80\%}    & \textbf{1.10\%}    & \textbf{1.00\%}     & \textbf{0.88\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ANLI\_r2\end{tabular}}} & \multicolumn{1}{l|}{1st Dropping} & 31.60\%         & 27.00\%            & 32.80\%             & 29.80\%            & 32.70\%            & 35.40\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 30.80\%         & 25.30\%            & 32.30\%             & 28.80\%            & 31.60\%            & 34.70\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{0.80\%} & \textbf{1.70\%}    & \textbf{0.50\%}     & \textbf{1.00\%}    & \textbf{1.10\%}    & \textbf{0.70\%}     & \textbf{0.97\%}          \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ANLI\_r3\end{tabular}}} & \multicolumn{1}{l|}{1st Dropping} & 33.08\%         & 26.75\%            & 32.75\%             & 30.50\%            & 35.92\%            & 38.75\%             &                          \\
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{2nd Dropping} & 32.67\%         & 26.33\%            & 32.17\%             & 29.58\%            & 35.42\%            & 38.08\%             &                          \\ \cmidrule(l){2-9} 
\multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{diff(-)}      & \textbf{0.42\%} & \textbf{0.42\%}    & \textbf{0.58\%}     & \textbf{0.92\%}    & \textbf{0.50\%}    & \textbf{0.67\%}     & \textbf{0.58\%}          \\ \midrule
\multicolumn{1}{l|}{Average}                                                                      &                                   &                 &                    &                     &                    &                    &                     & \textit{\textbf{1.64\%}} \\ \bottomrule
\end{tabular}
\caption{Proportion of instances left after each filter. On average, the second filter leads to $1.64\%$ instances of the full dataset getting dropped, which is negligible.}
\label{tab:dropprop}
\end{table*}

==> tables_adv/adv_trans_per_model.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Model Families} & \textbf{CIFAR10} & \textbf{CIFAR100} & \textbf{Oxford Flowers} & \textbf{Oxford Pets} \\ \midrule
AlexNet (Colorization, IN1K)     & 88.97 & 98.96 & 24.91 & 49.94 \\
AlexNet (Colorization, IN22K)    & 89.56 & 98.92 & 25.19 & 50.06 \\
AlexNet (Colorization, YFCC100M) & 87.84 & 98.55 & 24.91 & 49.96 \\
AlexNet (Jigsaw, IN1K)           & 53.25 & 74.03 & 26.96 & 45.38 \\
AlexNet (Jigsaw, IN22K)          & 53.06 & 73.76 & 30.61 & 49.86 \\
AlexNet (DeepCluster V2)         & 49.59 & 64.38 & 27.15 & 44.52 \\
ResNet-50 (Jigsaw, IN22K)        & 61.03 & 81.81 & 26.37 & 47.28 \\
ResNet-50 (Colorization, IN1K)   & 89.86 & 98.07 & 24.91 & 50.12 \\
ResNet-50 (Colorization, IN22K)  & 88.99 & 97.89 & 27.01 & 50.00 \\
ResNet-50 (Jigsaw, IN1K)         & 56.34 & 80.01 & 25.46 & 48.12 \\
ResNet-50 (Jigsaw, IN22K)        & 54.48 & 75.08 & 26.79 & 47.75 \\
ResNet-50 (RotNet, IN1K)         & 47.71 & 72.61 & 37.86 & 45.69 \\
ResNet-50 (Jigsaw, IN1K)         & 58.02 & 78.32 & 26.17 & 48.06 \\
ResNet-50 (NPID)                 & 58.37 & 80.39 & 49.77 & 48.42 \\
ResNet-50 (PIRL)                 & 58.80 & 84.12 & 34.03 & 44.10 \\
ResNet-101 (SimCLR)              & 55.09 & 70.34 & 28.54 & 47.12 \\
ResNet-50 (SimCLR)               & 51.57 & 65.91 & 30.26 & 44.12 \\
ResNet-50 (SwAV, 400ep)          & 48.63 & 68.46 & 28.79 & 44.33 \\
ResNet-50 (SwAV, 800ep)          & 50.23 & 67.89 & 27.73 & 45.33 \\
DeiT-Small (DINO)                & 63.37 & 85.08 & 26.56 & 47.26 \\
XCiT-Small (DINO)                & 49.46 & 64.84 & 27.19 & 46.76 \\
\bottomrule
\end{tabular}%
}
\caption{Adversarial Transferability Averaged for each dataset per model architecture type}
\label{tab:transferability_per_model}
\end{table}

==> tables_cqda/finetune_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
% \caption{MRR results for FOL queries on FB15K-237, with an unfrozen link predictor, i.e. complete model fine-tuning for \ours and CQD.}


%\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}=l+c+c+c+c+c+c+c+c+c+c+c+c@{}}
\toprule
\bf Model               & \bf 2p  & \bf 2i   & \bf 3i   & \bf pi   & \bf ip   & \bf 2u & \bf up & \bf 2in & \bf 3in & \bf inp & \bf pin & \bf pni \\ \midrule
%
%
%$\text{CQD}_{\text{fine-tuned}}$  & 8.0 & 20.8 & 34.8 & 18.5 & 13.7 & 9.7    & 6.5    & 5.0 & 7.1 & 4.5 & 2.6 & 2.2 \\
%$\text{\ours}_{\text{fine-tuned}}$ & 9.5 & 23.9 & 39.0 & 19.8 & 14.5 & 14.2   & 7.2    & 8.4 & 9.7 & 4.9 & 4.2 & 3.6 \\
%
%\midrule
%

% THIS ONE IS FOR THE REBUTTAL
% ./tools/results-cli.py logs/finetune_beaker_v1/*ds=fb237*freeze=True*neg=s*sf=none*.log
%CQD & 13.2 & 34.6 & 48.3 & 26.8 & 20.3 &   17.6 &   10.8 & 5.4 & 12.4 & 6.1 & 3.2 & 5.5 \\
%\rowstyle{\color{red}}
CQD & \bf 13.2 & 34.5 & 48.2 & 26.8 & 20.3 & 17.4 & 10.3 & 5.4 & 12.4 & 6.1 & 3.2 & 4.6 \\
% ./tools/results-cli.py logs/finetune_beaker_v1/*ds=fb237*freeze=False*sf=none*.log
CQD$_{\text{F}}$ &  9.3 & 22.8 & 34.9 & 19.8 & 14.5 &   13.0 &    7.2 & 7.4 & 7.1 & 4.9 & 3.9 & 3.8 \\
% ./tools/results-cli.py logs/finetune_beaker_v1/*ds=fb237*freeze=False*.log
CQD$^{\mathcal{A}}_{F}$ & 9.5 & 23.9 & 39.0 & 19.8 & 14.5 &   14.2 &    7.2 & 8.4 & 9.7 & 4.9 & 4.2 & 3.6 \\
% ./tools/results-cli.py logs/finetune_v4/*ds=fb237*freeze=True*pt=concat*.log
CQD$_{\text{C}}$ & 10.9 & 33.7 & 47.3 & 25.6 & 18.9 &   16.4 &    9.4 & 7.9 & 12.2 & 6.6 & 4.2 & 5.0 \\
% ./tools/results-cli.py logs/finetune_v4/*ds=fb237*freeze=True*pt=replace*.log 
CQD$_{\text{R}}$ & 6.4 & 22.2 & 31.0 & 16.6 & 11.2 &   12.5 &    4.8 & 4.7 & 5.9 & 4.1 & 2.0 & 3.5 \\
% ./tools/results-cli.py logs/finetune_beaker_v1/*ds=fb237*freeze=True*.log
\ours & \bf 13.2 & \bf 35.0 & \bf 48.5 & \bf 27.3 & \bf 20.7 &   \bf 17.6 &  \bf 10.5 & \bf 13.2 & \bf 14.9 & \bf 7.4 & \bf 7.8 & \bf 5.5 \\
\bottomrule
\end{tabular}%
%}
\caption{Test MRR results for FOL queries on FB15K-237 using the following CQD extensions: %\textcolor{red}
{CQD from \citet{DBLP:conf/iclr/ArakelyanDMC21,DBLP:conf/ijcai/MinerviniADC22} with the considered normalisation and negations;} CQD$_{\text{F}}$, where we fine-tune all neural link predictor parameters in CQD; CQD$^{\mathcal{A}}_{F}$, where we \emph{fine-tune all link predictor parameters} in \ours; CQD$_{\text{R}}$, where we learn a \emph{transformation} for the entity and relation embeddings and we use it to \emph{replace} the initial entity and relation representations; and CQD$_{\text{C}}$, where we learn a transformation for the entity and relation embeddings, and we \emph{concatenate} it to the initial entity and relation representations.}
\label{tab:fintetune_results}
\end{table*}

==> tables_cqda/stats.tex <==
\begin{table}[t]
\centering
\caption{Statistics on the different types of query structures in FB15K, FB15K-237, and NELL995.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
{\bf Split}                  & {\bf Query Type}     & {\bf FB15K}  & {\bf FB15K-237} & {\bf NELL995} \\ \midrule
\multirow{2}{*}{Training} & {1p}, {2p}, {3p}, {2i}, {3i}   & 273,710 & 149,689 & 107,982 \\
                       & {2in}, {3in}, {inp}, {pin}, {pni} & 27,371  & 14,968  & 10,798  \\ \midrule
\multirow{2}{*}{Validation} & {1p} & 59,078 & 20,094    & 16,910  \\
                       & Others         & 8,000  & 5,000     & 4,000   \\ \midrule
\multirow{2}{*}{Test}  & {1p} & 66,990 & 22,804    & 17,021  \\
                       & Others         & 8,000  & 5,000     & 4,000   \\ \bottomrule
\end{tabular}%
}
\label{tab:queries}
\end{table}

==> tables_flare/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

